Specification and Detection of LLM Code Smells

Large Language Models (LLMs) have gained massive popularity in recent years and are increasingly integrated into software systems for diverse purposes. However, poorly integrating them in source code may undermine software system quality. Yet, to our knowledge, there is no formal catalog of code smells specific to coding practices for LLM inference. In this paper, we introduce the concept of LLM code smells and formalize five recurrent problematic coding practices related to LLM inference in software systems, based on relevant literature. We extend the detection tool SpecDetect4AI to cover the newly defined LLM code smells and use it to validate their prevalence in a dataset of 200 open-source LLM systems. Our results show that LLM code smells affect 60.50% of the analyzed systems, with a detection precision of 86.06%.

==> Sections/Definition.tex <==


\textbf{LLM code smells} are code defects specific to the use of Large Language Models (LLMs) as software components within software systems. They correspond to problematic coding practices such as API misuse, incorrect hyperparameter settings, or inadequate handling of LLM inputs and outputs. Like other types of code smells ~\cite{10.5555/311424, badsmellsincode, Rivero2022CodeSmells, zhang2022codesmellsmachinelearning, gesi2022codesmellsmachinelearning, Carvalho2019AndroidSmells}, LLM Code Smells may not manifest as immediate bugs or failures, but they negatively affect software quality by impacting reliability, maintainability, and performance.

In summary, they can be characterized by three defining aspects:
\begin{itemize}
    \item They occur at the abstraction level of the source code.
    \item They are specific to the use of LLMs for inference as software components.
    \item They negatively affect the quality of the software system and its code.
\end{itemize}


% \textbf{LLM integration code smells} are code defects specific to the use of Large Language Models (LLMs) as software components within software systems. They correspond to problematic coding practices such as API misuse, incorrect hyperparameter settings, or inadequate handling of LLM inputs and outputs. Like other types of code smells ~\cite{10.5555/311424, badsmellsincode, Rivero2022CodeSmells, zhang2022codesmellsmachinelearning, gesi2022codesmellsmachinelearning, Carvalho2019AndroidSmells}, LLM Code Smells may not manifest as immediate bugs or failures, but they negatively affect software quality by impacting reliability, maintainability, and performance.

% In summary, they can be characterized by three defining aspects:
% \begin{itemize}
%     \item They occur at the abstraction level of the source code.
%     \item They are specific to the use of LLMs for inference as software components.
%     \item They negatively affect the quality of the software system and its code.
% \end{itemize}

